Demo Abstract: Fast Feedback Control and Coordination with Mode Changes for Wireless Cyber-Physical Systems

This abstract describes the first public demonstration of feedback control and coordination of multiple physical systems over a dynamic multi-hop low-power wireless network with update intervals of tens of milliseconds. Our running system can dynamically change between different sets of application tasks (e.g., sensing, actuation, control) executing on the spatially distributed embedded devices, while closed-loop stability is provably guaranteed even across those so-called mode changes. Moreover, any subset of the devices can move freely, which does not affect closed-loop stability and control performance as long as the wireless network remains connected.

==> requirements.tex <==
% !TEX root = paper.tex
\section*{Special Requirements}
\label{sec:requirements}

Our demo requires special equipment, as well as suitable locations for installing the wireless devices to form a three-hop network and for setting up the inverted pendulum systems.
Regarding space, we are already in touch with the General Chair of ACM/IEEE IPSN 2019 and CPS-IoT Week 2019, Prof.~Rasit Eskicioglu, who will provide us with further details on the conditions at the conference venue (floor plan, \etc).
As for special equipment, we will bring almost everything ourselves.
This is largely facilitated by generous support from the Canada-based manufacturer of the inverted pendulum systems we use, Quanser\footnote{\url{https://www.quanser.com/}}.
A Quanser engineer will help us set up the system on site over the weekend before the conference.
In addition, we will be shipping all our equipment to the Quanser headquaters in Markhand, ON, Canada in early March for careful testing of our demo setup.
This way, we aim to make sure that setting up and running our demo will be a smooth process.
Nevertheless, it would be great if the conference organizers could provide us with two large screens; otherwise, we will bring those with us, too.

 
